Towards Robust and Smooth 3D Multi-Person Pose Estimation from Monocular Videos in the Wild

3D pose estimation is an invaluable task in computer vision with various practical applications. Especially, 3D pose estimation for multi-person from a monocular video (3DMPPE) is particularly challenging and is still largely uncharted, far from applying to in-the-wild scenarios yet. We pose three unresolved issues with the existing methods: lack of robustness on unseen views during training, vulnerability to occlusion, and severe jittering in the output. As a remedy, we propose POTR-3D, the first realization of a sequence-to-sequence 2D-to-3D lifting model for 3DMPPE, powered by a novel geometry-aware data augmentation strategy, capable of generating unbounded data with a variety of views while caring about the ground plane and occlusions. Through extensive experiments, we verify that the proposed model and data augmentation robustly generalizes to diverse unseen views, robustly recovers the poses against heavy occlusions, and reliably generates more natural and smoother outputs. The effectiveness of our approach is verified not only by achieving the state-of-the-art performance on public benchmarks, but also by qualitative results on more challenging in-the-wild videos. Demo videos are available at https://www.youtube.com/@potr3d.

==> main_all.tex <==
@String(CVPR  = "Proc. of the IEEE/CVF Conference on Computer Vision and Pattern Recognition (CVPR)")
@String(ICCV  = "Proc. of the IEEE/CVF Conference on International Conference on Computer Vision (ICCV)")
@String(ECCV  = "Proc. of the European Conference on Computer Vision (ECCV)")
@String(BMVC  =	"Proc. of the British Machine Vision Conference (BMVC)")
@String(WACV  = "Pro. of the IEEE/CVF Winter Conference on Applications of Computer Vision (WACV)")
@String(NIPS  = "Advances in Neural Information Processing Systems (NIPS)")
@String(ICML  = "Proc. of the International Conference on Machine Learning (ICML)")
@String(ICLR  = "Proc. of the International Conference on Learning Representations (ICLR)")
@String(KDD   = "Proc. of the ACM SIGKDD International conference on knowledge discovery \& data mining")
@String(WWW   = "Proc. of the ACM International Conference on World Wide Web (WWW)")
@String(SIGIR = "Proc. of the International ACM Conference on Research and Development in Information Retrieval (SIGIR)")
@String(NAACL = "Proc. of the Conference of the North American Chapter of the Association for Computational Linguistics (NAACL)")


@String(PAMI  = {IEEE TPAMI})
@String(IJCV  = {IJCV})
@String(CVPR  = {CVPR})
@String(ICCV  = {ICCV})
@String(ECCV  = {ECCV})
@String(WACV  = {WACV})
@String(NIPS  = {NeurIPS})
@String(ICPR  = {ICPR})
@String(BMVC  =	{BMVC})
@String(TOG   = {ACM TOG})
@String(TIP   = {IEEE TIP})
@String(TVCG  = {IEEE TVCG})
@String(TCSVT = {IEEE TCSVT})
@String(TMM   =	{IEEE TMM})
@String(ACMMM = {ACM MM})
@String(ICME  =	{ICME})
@String(ICASSP=	{ICASSP})
@String(ICIP  = {ICIP})
@String(ACCV  = {ACCV})
@String(ICLR  = {ICLR})
@String(IJCAI = {IJCAI})
@String(PR = {PR})
@String(AAAI = {AAAI})
@String(CVPRW= {CVPRW})
@String(CSVT = {IEEE TCSVT})

@inproceedings{reddy2021tessetrack,
  title={Tesse{T}rack: End-to-End Learnable Multi-Person Articulated {3D} Pose Tracking},
  author={Reddy, N Dinesh and Guigues, Laurent and Pishchulin, Leonid and Eledath, Jayan and Narasimhan, Srinivasa G},
  booktitle={Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition},
  pages={15190--15200},
  year={2021}
}

@inproceedings{zanfir2018,
  title={Monocular {3D} pose and shape estimation of multiple people in natural scenes-the importance of multiple scene constraints.},
  author={Andrei Zanfir, Elisabeta Marinoiu, Cristian Sminchisescu},
  booktitle=CVPR,
  year={2018}
}

@article{zhang2022mixste,
  title={MixSTE: Seq2seq Mixed Spatio-Temporal Encoder for {3D} Human Pose Estimation in Video},
  author={Zhang, Jinlu and Tu, Zhigang and Yang, Jianyu and Chen, Yujin and Yuan, Junsong},
  journal={arXiv preprint arXiv:2203.00859},
  year={2022}
}


@article{llopart2020liftformer,
  title={Liftformer: {3D} human pose estimation using attention models},
  author={Llopart, Adrian},
  journal={arXiv preprint arXiv:2009.00348},
  year={2020}
}

@InProceedings{Cheng_2021_CVPR,
    author    = {Cheng, Yu and Wang, Bo and Yang, Bo and Tan, Robby T.},
    title     = {Monocular {3D} Multi-Person Pose Estimation by Integrating Top-Down and Bottom-Up Networks},
    booktitle = CVPR,
    year      = {2021}
}

@inproceedings{sun2019deep,
  title={Deep High-Resolution Representation Learning for Human Pose Estimation},
  author={Sun, Ke and Xiao, Bin and Liu, Dong and Wang, Jingdong},
  booktitle=CVPR,
  year={2019}
}

@inproceedings{zhang2022bytetrack,
  title={Byte{T}rack: Multi-Object Tracking by Associating Every Detection Box},
  author={Zhang, Yifu and Sun, Peize and Jiang, Yi and Yu, Dongdong and Weng, Fucheng and Yuan, Zehuan and Luo, Ping and Liu, Wenyu and Wang, Xinggang},
  booktitle=ECCV,
  year={2022}
}

@inproceedings{Wojke2018deep,
  title={Deep Cosine Metric Learning for Person Re-identification},
  author={Wojke, Nicolai and Bewley, Alex},
  booktitle=WACV,
  year={2018}
}

@inproceedings{pavllo20193d,
  title={{3D} human pose estimation in video with temporal convolutions and semi-supervised training},
  author={Pavllo, Dario and Feichtenhofer, Christoph and Grangier, David and Auli, Michael},
  booktitle=CVPR,
  year={2019}
}

@inproceedings{poseformerzheng20213d,
  title={{3D} human pose estimation with spatial and temporal transformers},
  author={Zheng, Ce and Zhu, Sijie and Mendieta, Matias and Yang, Taojiannan and Chen, Chen and Ding, Zhengming},
  booktitle=ICCV,
  year={2021}
}

@article{dosovitskiy2020image,
  title={An image is worth 16x16 words: Transformers for image recognition at scale},
  author={Dosovitskiy, Alexey and Beyer, Lucas and Kolesnikov, Alexander and Weissenborn, Dirk and Zhai, Xiaohua and Unterthiner, Thomas and Dehghani, Mostafa and Minderer, Matthias and Heigold, Georg and Gelly, Sylvain and others},
  journal={arXiv:2010.11929},
  year={2020}
}

@article{chen2021anatomy,
  title={Anatomy-aware {3D} human pose estimation with bone-based pose decomposition},
  author={Chen, Tianlang and Fang, Chen and Shen, Xiaohui and Zhu, Yiheng and Chen, Zhili and Luo, Jiebo},
  journal={IEEE Transactions on Circuits and Systems for Video Technology},
  volume={32},
  number={1},
  pages={198--209},
  year={2021},
  publisher={IEEE}
}

@inproceedings{vaswani2017attention,
  title={Attention is all you need},
  author={Vaswani, Ashish and Shazeer, Noam and Parmar, Niki and Uszkoreit, Jakob and Jones, Llion and Gomez, Aidan N and Kaiser, {\L}ukasz and Polosukhin, Illia},
  booktitle=NIPS,
  year={2017}
}

@inproceedings{liu2020attention,
  title={Attention mechanism exploits temporal contexts: Real-time {3D} human pose reconstruction},
  author={Liu, Ruixu and Shen, Ju and Wang, He and Chen, Chen and Cheung, Sen-ching and Asari, Vijayan},
  booktitle=CVPR,
  year={2020}
}

@inproceedings{sandler2018mobilenetv2,
  title={Mobile{N}etv2: Inverted residuals and linear bottlenecks},
  author={Sandler, Mark and Howard, Andrew and Zhu, Menglong and Zhmoginov, Andrey and Chen, Liang-Chieh},
  booktitle=CVPR,
  year={2018}
}

@inproceedings{chen2018cascaded,
  title={Cascaded pyramid network for multi-person pose estimation},
  author={Chen, Yilun and Wang, Zhicheng and Peng, Yuxiang and Zhang, Zhiqiang and Yu, Gang and Sun, Jian},
  booktitle=CVPR,
  year={2018}
}

@article{ye2021collaborative,
  title={Collaborative Refining for Person Re-Identification With Label Noise},
  author={Ye, Mang and Li, He and Du, Bo and Shen, Jianbing and Shao, Ling and Hoi, Steven CH},
  journal={IEEE Transactions on Image Processing},
  volume={31},
  pages={379--391},
  year={2021},
  publisher={IEEE}
}

@inproceedings{hossain2018exploiting,
  title={Exploiting temporal information for {3D} human pose estimation},
  author={Hossain, Mir Rayat Imtiaz and Little, James J},
  booktitle=ECCV,
  year={2018}
}

@inproceedings{joo2015panoptic,
    author = {Joo, Hanbyul and Liu, Hao and Tan, Lei and Gui, Lin and Nabbe, Bart and Matthews, Iain and Kanade, Takeo and Nobuhara, Shohei and Sheikh, Yaser},
    title = {Panoptic Studio: A Massively Multiview System for Social Motion Capture},
    booktitle = {ICCV},
    year = {2015} 
}

@article{sigal2010humaneva,
  title={Humaneva: Synchronized video and motion capture dataset and baseline algorithm for evaluation of articulated human motion},
  author={Sigal, Leonid and Balan, Alexandru O and Black, Michael J},
  journal={International journal of computer vision},
  volume={87},
  number={1},
  pages={4--27},
  year={2010},
  publisher={Springer}
}

@article{hochreiter1997long,
  title={Long short-term memory},
  author={Hochreiter, Sepp and Schmidhuber, J{\"u}rgen},
  journal={Neural computation},
  volume={9},
  number={8},
  pages={1735--1780},
  year={1997},
  publisher={MIT Press}
}

@inproceedings{mehta2017monocular,
  title={Monocular {3D} human pose estimation in the wild using improved cnn supervision},
  author={Mehta, Dushyant and Rhodin, Helge and Casas, Dan and Fua, Pascal and Sotnychenko, Oleksandr and Xu, Weipeng and Theobalt, Christian},
  booktitle={International conference on 3D vision (3DV)},
  year={2017}
}

@inproceedings{wang2020motion,
  title={Motion guided {3D} pose estimation from videos},
  author={Wang, Jingbo and Yan, Sijie and Xiong, Yuanjun and Lin, Dahua},
  booktitle=ECCV,
  year={2020}
}

@article{kingma2014adam,
  title={Adam: A method for stochastic optimization},
  author={Kingma, Diederik P and Ba, Jimmy},
  journal={arXiv:1412.6980},
  year={2014}
}

@article{ionescu2013human3,
  title={Human 3.6{M}: Large scale datasets and predictive methods for {3D} human sensing in natural environments},
  author={Ionescu, Catalin and Papava, Dragos and Olaru, Vlad and Sminchisescu, Cristian},
  journal={IEEE transactions on pattern analysis and machine intelligence},
  volume={36},
  number={7},
  pages={1325--1339},
  year={2013},
  publisher={IEEE}
}

@article{VirtualPose2022,
  title={{V}irtual{P}ose: Learning Generalizable 3D Human Pose Models from Virtual Data},
  author={Su, Jiajun and Wang, Chunyu and Ma, Xiaoxuan and Zeng, Wenjun and Wang, Yizhou},
  journal={arXiv:2207.09949},
  year={2022}
}

@InProceedings{Jin_2022_CVPR,
    author    = {Jin, Lei and Xu, Chenyang and Wang, Xiaojuan and Xiao, Yabo and Guo, Yandong and Nie, Xuecheng and Zhao, Jian},
    title     = {Single-Stage Is Enough: Multi-Person Absolute {3D} Pose Estimation},
    booktitle = CVPR,
    year      = {2022}
}

@inproceedings{zhang2018mask,
  title={Mask {R-CNN} with feature pyramid attention for instance segmentation},
  author={Zhang, Xiangyi and An, Gaoyun and Liu, Yutian},
  booktitle={Proc. of the IEEE International Conference on Signal Processing (ICSP)},
  year={2018}
}

@inproceedings{ramakrishna2012reconstructing,
  title={Reconstructing {3D} human pose from {2D} image landmarks},
  author={Ramakrishna, Varun and Kanade, Takeo and Sheikh, Yaser},
  booktitle=ECCV,
  year={2012}
}

@book{hartley2003multiple,
  title={Multiple view geometry in computer vision},
  author={Hartley, Richard and Zisserman, Andrew},
  year={2003},
  publisher={Cambridge university press}
}

@inproceedings{joo2019towards,
  title={Towards social artificial intelligence: Nonverbal social signal prediction in a triadic interaction},
  author={Joo, Hanbyul and Simon, Tomas and Cikara, Mina and Sheikh, Yaser},
  booktitle=CVPR,
  year={2019}
}

@inproceedings{bridgeman2019multi,
  title={Multi-person {3D} pose estimation and tracking in sports},
  author={Bridgeman, Lewis and Volino, Marco and Guillemaut, Jean-Yves and Hilton, Adrian},
  booktitle={CVPR Workshops},
  year={2019}
}
@inproceedings{dong2019fast,
  title={Fast and robust multi-person {3D} pose estimation from multiple views},
  author={Dong, Junting and Jiang, Wen and Huang, Qixing and Bao, Hujun and Zhou, Xiaowei},
  booktitle={Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition},
  pages={7792--7801},
  year={2019}
}

@inproceedings{amin2013multi,
  title={Multi-view pictorial structures for {3D} human pose estimation.},
  author={Amin, Sikandar and Andriluka, Mykhaylo and Rohrbach, Marcus and Schiele, Bernt},
  booktitle={Bmvc},
  volume={1},
  number={2},
  year={2013}
}
@inproceedings{pishchulin2016deepcut,
  title={Deepcut: Joint subset partition and labeling for multi person pose estimation},
  author={Pishchulin, Leonid and Insafutdinov, Eldar and Tang, Siyu and Andres, Bjoern and Andriluka, Mykhaylo and Gehler, Peter V and Schiele, Bernt},
  booktitle={Proceedings of the IEEE conference on computer vision and pattern recognition},
  pages={4929--4937},
  year={2016}
}
@inproceedings{moreno20173d,
  title={{3D} human pose estimation from a single image via distance matrix regression},
  author={Moreno-Noguer, Francesc},
  booktitle={Proceedings of the IEEE Conference on Computer Vision and Pattern Recognition},
  pages={2823--2832},
  year={2017}
}

@inproceedings{martinez2017simple,
  title={A simple yet effective baseline for {3D} human pose estimation},
  author={Martinez, Julieta and Hossain, Rayat and Romero, Javier and Little, James J},
  booktitle=ICCV,
  year={2017}
}

@inproceedings{qiu2019cross,
  title={Cross view fusion for {3D} human pose estimation},
  author={Qiu, Haibo and Wang, Chunyu and Wang, Jingdong and Wang, Naiyan and Zeng, Wenjun},
  booktitle=ICCV,
  year={2019}
}

@inproceedings{iskakov2019learnable,
  title={Learnable triangulation of human pose},
  author={Iskakov, Karim and Burkov, Egor and Lempitsky, Victor and Malkov, Yury},
  booktitle=ICCV,
  year={2019}
}

@inproceedings{pavlakos2018ordinal,
  title={Ordinal depth supervision for {3D} human pose estimation},
  author={Pavlakos, Georgios and Zhou, Xiaowei and Daniilidis, Kostas},
  booktitle=CVPR,
  year={2018}
}

@inproceedings{zhou2017towards,
  title={Towards {3D} human pose estimation in the wild: a weakly-supervised approach},
  author={Zhou, Xingyi and Huang, Qixing and Sun, Xiao and Xue, Xiangyang and Wei, Yichen},
  booktitle=ICCV,
  year={2017}
}

@inproceedings{cheng20203d,
  title={{3D} human pose estimation using spatio-temporal networks with explicit occlusion training},
  author={Cheng, Yu and Yang, Bo and Wang, Bo and Tan, Robby T},
  booktitle=AAAI,
  year={2020}
}

@inproceedings{cheng2019occlusion,
  title={Occlusion-aware networks for {3D} human pose estimation in video},
  author={Cheng, Yu and Yang, Bo and Wang, Bo and Yan, Wending and Tan, Robby T},
  booktitle=ICCV,
  year={2019}
}

@inproceedings{carion2020end,
  title={End-to-end object detection with transformers},
  author={Carion, Nicolas and Massa, Francisco and Synnaeve, Gabriel and Usunier, Nicolas and Kirillov, Alexander and Zagoruyko, Sergey},
  booktitle=ECCV,
  year={2020}
}

@inproceedings{yang2020transpose,
  title={Transpose: Keypoint localization via transformer},
  author={Yang, Sen and Quan, Zhibin and Nie, Mu and Yang, Wankou},
  booktitle=ICCV,
  year={2021}
}

@inproceedings{lin2021end,
  title={End-to-end human pose and mesh reconstruction with transformers},
  author={Lin, Kevin and Wang, Lijuan and Liu, Zicheng},
  booktitle=CVPR,
  year={2021}
}

@inproceedings{he2020epipolar,
  title={Epipolar transformers},
  author={He, Yihui and Yan, Rui and Fragkiadaki, Katerina and Yu, Shoou-I},
  booktitle=CVPR,
  year={2020}
}

@article{li2022exploiting,
  title={Exploiting temporal contexts with strided transformer for {3D} human pose estimation},
  author={Li, Wenhao and Liu, Hong and Ding, Runwei and Liu, Mengyuan and Wang, Pichao and Yang, Wenming},
  journal={IEEE Transactions on Multimedia},
  year={2022},
  publisher={IEEE}
}

@inproceedings{mscoco,
  title={Microsoft {COCO}: Common objects in context},
  author={Lin, Tsung-Yi and Maire, Michael and Belongie, Serge and Hays, James and Perona, Pietro and Ramanan, Deva and Doll{\'a}r, Piotr and Zitnick, C Lawrence},
  booktitle=ECCV,
  year={2014}
}

@inproceedings{mono-3dhp2017,
 author = {Mehta, Dushyant and Rhodin, Helge and Casas, Dan and Fua, Pascal and Sotnychenko, Oleksandr and Xu, Weipeng and Theobalt, Christian},
 title = {Monocular {3D} Human Pose Estimation In The Wild Using Improved CNN Supervision},
 booktitle = {3D Vision (3DV), 2017 Fifth International Conference on},
 year = {2017},
 organization={IEEE}
}

@inproceedings{singleshotmultiperson2018,
title = {Single-Shot Multi-Person {3D} Pose Estimation From Monocular RGB},
author = {Mehta, Dushyant and Sotnychenko, Oleksandr and Mueller, Franziska and Xu, Weipeng and Sridhar, Srinath and Pons-Moll, Gerard and Theobalt, Christian},
booktitle = {3D Vision (3DV), 2018 Sixth International Conference on},
year = {2018},
organization={IEEE}
} 

@inproceedings{tu2020voxelpose,
  title={Voxel{P}ose: Towards multi-camera {3D} human pose estimation in wild environment},
  author={Tu, Hanyue and Wang, Chunyu and Zeng, Wenjun},
  booktitle=ECCV,
  year={2020}
}


@inproceedings{CLIPradford2021learning,
  title={Learning transferable visual models from natural language supervision},
  author={Radford, Alec and Kim, Jong Wook and Hallacy, Chris and Ramesh, Aditya and Goh, Gabriel and Agarwal, Sandhini and Sastry, Girish and Askell, Amanda and Mishkin, Pamela and Clark, Jack and others},
  booktitle=ICML,
  year={2021}
}

@inproceedings{GPT-3brown2020language,
  title={Language models are few-shot learners},
  author={Brown, Tom and Mann, Benjamin and Ryder, Nick and Subbiah, Melanie and Kaplan, Jared D and Dhariwal, Prafulla and Neelakantan, Arvind and Shyam, Pranav and Sastry, Girish and Askell, Amanda and others},
  booktitle=NIPS,
  year={2020}
}

@inproceedings{Rogez_2017_CVPR,
  author = {Rogez, Gregory and Weinzaepfel, Philippe and Schmid, Cordelia},
  title = {{LCR-N}et: Localization-Classification-Regression for Human Pose},
  booktitle = CVPR,
  year = {2017}
}

@inproceedings{Moon_2019_ICCV_3DMPPE,
  author = {Moon, Gyeongsik and Chang, Juyong and Lee, Kyoung Mu},
  title = {Camera Distance-aware Top-down Approach for {3D} Multi-person Pose Estimation from a Single RGB Image},
 booktitle = ICCV,
  year = {2019}
}

@inproceedings{nie2019single,
  title={Single-stage multi-person pose machines},
  author={Nie, Xuecheng and Feng, Jiashi and Zhang, Jianfeng and Yan, Shuicheng},
  booktitle=ICCV,
  year={2019}
}

@inproceedings{zanfir2018deep,
  title={Deep network for the integrated {3D} sensing of multiple people in natural images},
  author={Zanfir, Andrei and Marinoiu, Elisabeta and Zanfir, Mihai and Popa, Alin-Ionut and Sminchisescu, Cristian},
  booktitle=NIPS,
  year={2018}
}

@inproceedings{kundu2020unsupervised,
  title={Unsupervised cross-modal alignment for multi-person {3D} pose estimation},
  author={Kundu, Jogendra Nath and Revanur, Ambareesh and Waghmare, Govind Vitthal and Venkatesh, Rahul Mysore and Babu, R Venkatesh},
  booktitle=ECCV,
  year={2020}
}

@inproceedings{chen2017enhancing,
  title={Enhancing detection model for multiple hypothesis tracking},
  author={Chen, Jiahui and Sheng, Hao and Zhang, Yang and Xiong, Zhang},
  booktitle={CVPR Workshops},
  year={2017}
}

@inproceedings{bewley2016simple,
  title={Simple online and realtime tracking},
  author={Bewley, Alex and Ge, Zongyuan and Ott, Lionel and Ramos, Fabio and Upcroft, Ben},
  booktitle={Proc. of the IEEE international conference on image processing (ICIP)},
  year={2016}
}

@article{SMPL:2015,
      author = {Loper, Matthew and Mahmood, Naureen and Romero, Javier and Pons-Moll, Gerard and Black, Michael J.},
      title = {{SMPL}: A Skinned Multi-Person Linear Model},
      journal = {ACM Trans. Graphics (Proc. SIGGRAPH Asia)},
      month = oct,
      number = {6},
      pages = {248:1--248:16},
      publisher = {ACM},
      volume = {34},
      year = {2015}
    }

@misc{facevid2vidnvidia,
  doi = {10.48550/ARXIV.2011.15126},
  
  url = {https://arxiv.org/abs/2011.15126},
  
  author = {Wang, Ting-Chun and Mallya, Arun and Liu, Ming-Yu},
  
  keywords = {Computer Vision and Pattern Recognition (cs.CV), FOS: Computer and information sciences, FOS: Computer and information sciences},
  
  title = {One-Shot Free-View Neural Talking-Head Synthesis for Video Conferencing},
  
  publisher = {arXiv},
  
  year = {2020},
  
  copyright = {arXiv.org perpetual, non-exclusive license}
}

@article{mahmoudi2019multi,
  title={Multi-target tracking using CNN-based features: {CNNMTT}},
  author={Mahmoudi, Nima and Ahadi, Seyed Mohammad and Rahmati, Mohammad},
  journal={Multimedia Tools and Applications},
  volume={78},
  number={6},
  pages={7077--7096},
  year={2019},
  publisher={Springer}
}

@inproceedings{kim2018multi,
  title={Multi-object tracking with neural gating using bilinear lstm},
  author={Kim, Chanho and Li, Fuxin and Rehg, James M},
  booktitle=ECCV,
  year={2018}
}

@article{kalman1960new,
  title={A new approach to linear filtering and prediction problems},
  author={Kalman, Rudolph Emil},
  year={1960}
}

@article{wang2017robust,
  title={Robust tracking of fish schools using CNN for head identification},
  author={Wang, Shuo Hong and Zhao, Jing Wen and Chen, Yan Qiu},
  journal={Multimedia Tools and Applications},
  volume={76},
  number={22},
  pages={23679--23697},
  year={2017},
  publisher={Springer}
}

@inproceedings{wang2017online,
  title={Online multiple object tracking via flow and convolutional features},
  author={Wang, Lu and Xu, Lisheng and Kim, Min Young and Rigazico, Luca and Yang, Ming-Hsuan},
  booktitle={IEEE International Conference on Image Processing (ICIP)},
  year={2017}
}

@inproceedings{rosello2018multi,
  title={Multi-agent reinforcement learning for multi-object tracking},
  author={Rosello, Pol and Kochenderfer, Mykel J},
  booktitle={Proc. of the International Conference on Autonomous Agents and MultiAgent Systems},
  year={2018}
}

@inproceedings{he2016deep,
  title={Deep residual learning for image recognition},
  author={He, Kaiming and Zhang, Xiangyu and Ren, Shaoqing and Sun, Jian},
  booktitle=CVPR,
  year={2016}
}

@inproceedings{detr2020,
  title={End-to-end object detection with transformers},
  author={Carion, Nicolas and Massa, Francisco and Synnaeve, Gabriel and Usunier, Nicolas and Kirillov, Alexander and Zagoruyko, Sergey},
  booktitle=ECCV,
  year={2020}
}

@article{kipf2016semi,
  title={Semi-supervised classification with graph convolutional networks},
  author={Kipf, Thomas N and Welling, Max},
  journal={arXiv:1609.02907},
  year={2016}
}

@inproceedings{cai2019exploiting,
  title={Exploiting spatial-temporal relationships for {3D} pose estimation via graph convolutional networks},
  author={Cai, Yujun and Ge, Liuhao and Liu, Jun and Cai, Jianfei and Cham, Tat-Jen and Yuan, Junsong and Thalmann, Nadia Magnenat},
  booktitle=ICCV,
  year={2019}
}

@inproceedings{lin2017recurrent,
  title={Recurrent {3D} pose sequence machines},
  author={Lin, Mude and Lin, Liang and Liang, Xiaodan and Wang, Keze and Cheng, Hui},
  booktitle=CVPR,
  year={2017}
}

@inproceedings{gong2021poseaug,
  title={Pose{A}ug: A differentiable pose augmentation framework for {3D} human pose estimation},
  author={Gong, Kehong and Zhang, Jianfeng and Feng, Jiashi},
  booktitle=CVPR,
  year={2021}
}

@inproceedings{gholami2022adaptpose,
  title={Adapt{P}ose: Cross-Dataset Adaptation for {3D} Human Pose Estimation by Learnable Motion Generation},
  author={Gholami, Mohsen and Wandt, Bastian and Rhodin, Helge and Ward, Rabab and Wang, Z Jane},
  booktitle=CVPR,
  year={2022}
}

@article{kanade1997virtualized,
  title={Virtualized reality: Constructing virtual worlds from real scenes},
  author={Kanade, Takeo and Rander, Peter and Narayanan, PJ},
  journal={IEEE multimedia},
  volume={4},
  number={1},
  pages={34--47},
  year={1997},
  publisher={IEEE}
}

@inproceedings{wu2020human,
  title={Human {3D} pose estimation in a lying position by RGB-D images for medical diagnosis and rehabilitation},
  author={Wu, Qingqiang and Xu, Guanghua and Zhang, Sicong and Li, Yu and Wei, Fan},
  booktitle={Annual International Conference of the IEEE Engineering in Medicine \& Biology Society (EMBC)},
  year={2020}
}

@inproceedings{ke2010real,
  title={Real-time {3D} human pose estimation from monocular view with applications to event detection and video gaming},
  author={Ke, Shian-Ru and Zhu, LiangJia and Hwang, Jenq-Neng and Pai, Hung-I and Lan, Kung-Ming and Liao, Chih-Pin},
  booktitle={Proc. of the IEEE International Conference on Advanced Video and Signal Based Surveillance},
  year={2010}
}

@inproceedings{alahari2013pose,
  title={Pose estimation and segmentation of people in 3D movies},
  author={Alahari, Karteek and Seguin, Guillaume and Sivic, Josef and Laptev, Ivan},
  booktitle=ICCV,
  year={2013}
}

@article{Lu2019vilbert,
  title={{V}il{BERT}: Pretraining task-agnostic visiolinguistic representations for vision-and-language tasks},
  author={Lu, Jiasen and Batra, Dhruv and Parikh, Devi and Lee, Stefan},
  journal=NIPS,
  volume={32},
  year={2019}
}

@inproceedings{Sun2019videobert,
  title={Video{BERT}: A joint model for video and language representation learning},
  author={Sun, Chen and Myers, Austin and Vondrick, Carl and Murphy, Kevin and Schmid, Cordelia},
  booktitle=ICCV,
  year={2019}
}

@article{Zhang2020hammer,
  title={A hierarchical multi-modal encoder for moment localization in video corpus},
  author={Zhang, Bowen and Hu, Hexiang and Lee, Joonseok and Zhao, Ming and Chammas, Sheide and Jain, Vihan and Ie, Eugene and Sha, Fei},
  journal={arXiv:2011.09046},
  year={2020}
}

@inproceedings{arnab2021vivit,
  title={Vi{V}it: A video vision transformer},
  author={Arnab, Anurag and Dehghani, Mostafa and Heigold, Georg and Sun, Chen and Lu{\v{c}}i{\'c}, Mario and Schmid, Cordelia},
  booktitle=ICCV,
  year={2021}
}

@article{hofmann2012multi,
  title={Multi-view {3D} human pose estimation in complex environment},
  author={Hofmann, Michael and Gavrila, Dariu M},
  journal={International journal of computer vision},
  volume={96},
  number={1},
  pages={103--124},
  year={2012},
  publisher={Springer}
}

@inproceedings{remelli2020lightweight,
  title={Lightweight multi-view 3d pose estimation through camera-disentangled representation},
  author={Remelli, Edoardo and Han, Shangchen and Honari, Sina and Fua, Pascal and Wang, Robert},
  booktitle=CVPR,
  year={2020}
}

@inproceedings{hofmann2009multi,
  title={Multi-view {3D} human pose estimation combining single-frame recovery, temporal integration and model adaptation},
  author={Hofmann, Michael and Gavrila, Dariu M},
  booktitle=CVPR,
  year={2009}
}

@inproceedings{zhang2021direct,
  title={Direct multi-view multi-person 3d pose estimation},
  author={Zhang, Jianfeng and Cai, Yujun and Yan, Shuicheng and Feng, Jiashi and others},
  booktitle=NIPS,
  year={2021}
}

@article{bultmann2021real,
  title={Real-time multi-view {3D} human pose estimation using semantic feedback to smart edge sensors},
  author={Bultmann, Simon and Behnke, Sven},
  journal={arXiv:2106.14729},
  year={2021}
}

@inproceedings{newell2016stacked,
  title={Stacked hourglass networks for human pose estimation},
  author={Newell, Alejandro and Yang, Kaiyu and Deng, Jia},
  booktitle=ECCV,
  year={2016}
}

@article{wang2020deep,
  title={Deep high-resolution representation learning for visual recognition},
  author={Wang, Jingdong and Sun, Ke and Cheng, Tianheng and Jiang, Borui and Deng, Chaorui and Zhao, Yang and Liu, Dong and Mu, Yadong and Tan, Mingkui and Wang, Xinggang and others},
  journal={IEEE transactions on pattern analysis and machine intelligence},
  volume={43},
  number={10},
  pages={3349--3364},
  year={2020},
  publisher={IEEE}
}

@inproceedings{wei2016convolutional,
  title={Convolutional pose machines},
  author={Wei, Shih-En and Ramakrishna, Varun and Kanade, Takeo and Sheikh, Yaser},
  booktitle=CVPR,
  year={2016}
}

@inproceedings{xiao2018simple,
  title={Simple baselines for human pose estimation and tracking},
  author={Xiao, Bin and Wu, Haiping and Wei, Yichen},
  booktitle=ECCV,
  year={2018}
}

@article{wang2021survey,
  title={Deep {3D} human pose estimation: A review},
  author={Wang, Jinbao and Tan, Shujie and Zhen, Xiantong and Xu, Shuo and Zheng, Feng and He, Zhenyu and Shao, Ling},
  journal={Computer Vision and Image Understanding},
  volume={210},
  pages={103225},
  year={2021},
  publisher={Elsevier}
}

@article{gamra2021review,
  title={A review of deep learning techniques for {2D} and {3D} human pose estimation},
  author={Gamra, Miniar Ben and Akhloufi, Moulay A},
  journal={Image and Vision Computing},
  volume={114},
  pages={104282},
  year={2021},
  publisher={Elsevier}
}

@inproceedings{zhao2019semantic,
  title={Semantic graph convolutional networks for 3d human pose regression},
  author={Zhao, Long and Peng, Xi and Tian, Yu and Kapadia, Mubbasir and Metaxas, Dimitris N},
  booktitle=CVPR,
  year={2019}
}

@inproceedings{liu2020comprehensive,
  title={A comprehensive study of weight sharing in graph networks for 3d human pose estimation},
  author={Liu, Kenkun and Ding, Rongqi and Zou, Zhiming and Wang, Le and Tang, Wei},
  booktitle=ECCV,
  year={2020}
}

@inproceedings{ci2019optimizing,
  title={Optimizing network structure for 3d human pose estimation},
  author={Ci, Hai and Wang, Chunyu and Ma, Xiaoxuan and Wang, Yizhou},
  booktitle=ICCV,
  year={2019}
}

@inproceedings{li2022mhformer,
  title={Mhformer: Multi-hypothesis transformer for 3d human pose estimation},
  author={Li, Wenhao and Liu, Hong and Tang, Hao and Wang, Pichao and Van Gool, Luc},
  booktitle={Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition},
  pages={13147--13156},
  year={2022}
}
 @misc{intel, title={Intel® 3D athlete tracking - markerless motion capture}, url={https://www.intel.com/content/www/us/en/architecture-and-technology/3d-athlete-tracking.html}, journal={Intel}} 

 @inproceedings{zhen2020smap,
  title={Smap: Single-shot multi-person absolute 3d pose estimation},
  author={Zhen, Jianan and Fang, Qi and Sun, Jiaming and Liu, Wentao and Jiang, Wei and Bao, Hujun and Zhou, Xiaowei},
  booktitle={European Conference on Computer Vision},
  pages={550--566},
  year={2020},
  organization={Springer}
}

==> tab/result_2.tex <==



\begin{table}
\resizebox{\linewidth}{!}{ %< auto-adjusts font size to fill line
    \centering
    \begin{tabular}{cccc|c|c|cccc}
    \toprule
    PT & PR & GPT & GPR & Model & Size & PCK$_\text{rel}$(\%)$\uparrow$ & PCK$_\text{abs}$(\%)$\uparrow$ & MPJVE$_\text{rel}$(mm)$\downarrow$ & MPJVE$_\text{abs}$(mm)$\downarrow$ \\ 
    \midrule
    & & & & B & 0.4M  &  80.2     & 37.8      & 10.9  & 17.0 \\
    \checkmark & & & & B & 0.7M  &  82.8     & 40.6      & 11.4  & 18.7 \\
    & & & & B & 1.3M  &  82.8     & 40.9      & 10.9  & 16.8 \\
    \midrule
    \checkmark & & & & \sungchan{L} & \sungchan{1.3M}  &      &    &   &  \\
    \midrule
    & & & & B & 0.4M  &  81.0     & 41.3      & 11.0  & 16.7 \\
    \checkmark & \checkmark & & & B & 0.7M  &  83.7     & \textbf{50.9}      & 10.9  & \textbf{16.3} \\
    & & & & B & 1.3M  &  83.0     & 47.1      & 10.8  & 18.1 \\
    \midrule
    \checkmark & \checkmark & & & \sungchan{L} & \sungchan{1.3M}  &      &    &   &  \\
    \midrule
    & & & & B & 0.4M  &  82.3     & 42.1      & 10.9  & 17.1 \\
    \checkmark & \checkmark & \checkmark & & B & 0.7M  &  82.2     & 45.9      & \textbf{10.7}  & 17.0 \\
    & & &  & B & 1.3M  &  83.7     & 45.4      & \textbf{10.7}  & 18.7 \\
    \midrule
    \checkmark & \checkmark & \checkmark & & \sungchan{L} & \sungchan{1.3M}  &      &    &   &  \\
    \midrule
    & & & & B & 0.4M  &  81.3     & 41.9      & 11.2  & 17.1 \\
    \checkmark & \checkmark & \checkmark & \checkmark & B & 0.7M  &  83.3     & 48.1      & 10.8  & 18.3 \\
    & & & & B & 1.3M  &  \textbf{84.3}     & 46.1     & 11.0  & 16.5 \\
    \midrule
    \checkmark & \checkmark & \checkmark & \checkmark & \sungchan{L} & \sungchan{1.3M}  &      &    &   &  \\
    \bottomrule
    \end{tabular}
} % \resizebox
    %\vspace{-0.2cm}
    \caption{
        \textbf{Ablation Study on Augmentation Strategy on MuPoTS-3D.} The best scores are marked in boldface.
    } % \caption
    \label{tab:ablation_mupots}
    %\vspace{-0.2cm}
\end{table}


==> tab/result_pano_2.tex <==
\begin{table}
\resizebox{\linewidth}{!}{ %< auto-adjusts font size to fill line
    \centering
    \begin{tabular}{cccc|c|cc}
    \toprule
    PT & PR & GPT & GPR &
    Size                                &
    MPJPE$_\text{rel}$(mm)$\downarrow$  & MPJVE$_\text{rel}$(mm)$\downarrow$ \\
    \midrule
    \midrule
    \checkmark & & &
        & 0.5M
        & 87.1
        & 4.5\\
    \checkmark & \checkmark & &
        & 0.5M
        & \textbf{58.3}
        & 4.6\\
    \checkmark & \checkmark & \checkmark &
        & 0.5M
        & 58.5
        & 5.0\\
    \checkmark & \checkmark & \checkmark & \checkmark
        & 0.5M
        & 72.7
        & 4.8\\
    \midrule
    \checkmark & \checkmark & \checkmark & \checkmark
        & 0.8M
        & 68.8
        & \textbf{4.2} \\
    \bottomrule
    \end{tabular}
} % \resizebox
\vspace{-0.2cm}
\caption{
    \textbf{Ablation Study on Augmentation Strategy on CMU-Panoptic.} The best scores are marked in boldface.
} % \caption
\label{tab:ablation_panotic}
\vspace{-0.3cm}
\end{table}
